Queueing, Predictions, and LLMs: Challenges and Open Problems

Queueing systems present many opportunities for applying machine-learning predictions, such as estimated service times, to improve system performance. This integration raises numerous open questions about how predictions can be effectively leveraged to improve scheduling decisions. Recent studies explore queues with predicted service times, typically aiming to minimize job time in the system. We review these works, highlight the effectiveness of predictions, and present open questions on queue performance. We then move to consider an important practical example of using predictions in scheduling, namely Large Language Model (LLM) systems, which presents novel scheduling challenges and highlights the potential for predictions to improve performance. In particular, we consider LLMs performing inference. Inference requests (jobs) in LLM systems are inherently complex; they have variable inference times, dynamic memory footprints that are constrained by key-value (KV) store memory limitations, and multiple possible preemption approaches that affect performance differently. We provide background on the important aspects of scheduling in LLM systems, and introduce new models and open problems that arise from them. We argue that there are significant opportunities for applying insights and analysis from queueing theory to scheduling in LLM systems.

==> removed.tex <==
\section{Introduction}

Queueing systems have traditionally focused on analyzing and optimizing metrics such as average waiting time and overall system latency. These analyses are typically based on exact or stochastic job service times. 
Machine learning has enabled service time prediction, leading to more advanced scheduling algorithms. These capabilities allow schedulers to make better-informed decisions, significantly improving performance metrics, especially in systems with high variability and uncertainty. Studies in this area have demonstrated that leveraging predictions can lead to better scheduling policies that outperform traditional approaches, especially in systems with high variability and uncertainty. The intersection between machine learning and traditional algorithms in general, and queueing theory in particular, has led to the rise of algorithms with predictions, also known as learning-augmented algorithms, where classical algorithms are enhanced by incorporating advice or predictions from machine learning models or other sources. These learning-augmented algorithms have demonstrated their effectiveness across a range of areas~\cite{}.



%mention type of predictions and challenges, different types and cost, that lead to open questions that we are stating here


%here start to talk about LLM
\subsection{OLD intro}
Machine learning research is advancing rapidly, reshaping numerous fields and presenting new opportunities for optimization. The intersection between machine learning and traditional algorithms has led to the rise of algorithms with predictions, also known as learning-augmented algorithms, where classical algorithms are enhanced by incorporating advice or predictions from machine learning models or other sources. These learning-augmented algorithms have demonstrated their effectiveness across a range of areas~\cite{}.

Queueing systems are an example in which the learning-augmented algorithm paradigm has been applied, particularly in the context of scheduling. Several studies have examined queues that utilize predicted service times instead of exact ones, generally aiming to minimize the average time a job spends in the system.

Predictions can take various forms, each comes with its own challenges and costs. For example, when predicting job sizes, we might frame the prediction as a classification problem (determining whether a job is short or long), as an exact value (an absolute size), or as a probability distribution.



\begin{itemize}
    \item 
Set the Context: Begin by highlighting the significance of queueing and scheduling in computational systems, and how predictive algorithms have advanced this field.

    \item 
Motivation: Explain why LLM systems present unique challenges for queueing and scheduling, emphasizing the importance of efficient resource management due to their computational intensity.

    \item 
Objectives and Contributions: Clearly state the goals of your paper, including the survey of existing algorithms, identification of challenges, and presentation of open questions specific to LLM applications.

\end{itemize}



Machine learning research is advancing rapidly, reshaping many fields and presenting opportunities for optimization. 


Queueing systems have seen significant advancements through the integration of machine learning techniques. Traditionally, queueing theory has focused on analyzing and optimizing systems based on exact or stochastic models of service times and arrival processes. However, the advent of machine learning has enabled the prediction of service times and the development of more sophisticated scheduling algorithms. This shift represents a paradigm where machine learning is not just an application area for queueing theory but also a tool to enhance and refine queueing models themselves.

In classical queueing systems, the primary objective has often been to minimize metrics such as the average waiting time or overall system latency. With the incorporation of predicted service times, schedulers can make more informed decisions, potentially improving performance metrics significantly. Studies in this area have demonstrated that leveraging predictions can lead to better scheduling policies that outperform traditional approaches, especially in systems with high variability and uncertainty.

The emergence of Large Language Models (LLMs), such as GPT-3 and GPT-4, has introduced a new set of challenges and opportunities in the context of queueing and scheduling. LLMs are computationally intensive models that require substantial resources for both training and inference. Here, we focus on inference time, where these models must handle a diverse and complex set of requests with varying computational demands. Unlike traditional jobs in queueing systems, requests to LLMs can have highly variable inference times due to differences in response lengths.

Moreover, LLM systems often operate under constraints that were not prevalent in traditional queueing models. For instance, the key-value (KV) memory limitations inherent in transformer architectures introduce dynamic memory footprints that can affect how jobs are scheduled and executed. Preemption, a common strategy in scheduling, becomes more complicated when dealing with stateful models that maintain context across interactions. Additionally, performance metrics have expanded beyond mere latency to include cost considerations, such as energy consumption, and qualitative aspects like the accuracy and usefulness of the generated responses.

These complexities necessitate the development of new queueing models and scheduling algorithms tailored to the specific needs of LLM systems. There is a pressing need for research that bridges the gap between queueing theory and the practical requirements of deploying LLMs in real-world applications. This paper seeks to address this need by providing a comprehensive survey of existing algorithms that incorporate predictions for scheduling and by identifying open problems unique to LLM applications.

We aim to introduce queueing theorists to the intricacies of LLM systems, highlighting how traditional models can be extended or adapted to accommodate the challenges they present. By examining the interplay between predicted service times and the unique characteristics of LLM workloads, we hope to inspire new research directions that will lead to more efficient and effective scheduling policies.

The remainder of this paper is structured as follows:





Section 2 reviews the current state of scheduling with job size predictions, discussing how machine learning techniques have been employed to improve queueing performance.



Section 3 defines the specific challenges posed by LLM systems, including inference time scheduling, KV memory limitations, and the impact of preemption on performance metrics such as runtime, cost, and accuracy.



Section 4 focuses on the case of a single LLM, exploring how traditional queueing models can be adapted to address the unique characteristics of LLM inference workloads.



Section 5 examines scenarios involving LLMs with agents, considering the additional complexities introduced by multi-agent interactions and shared resources.



Section 6 discusses distributed LLM systems, delving into load balancing strategies that account for computational load, attention mechanisms, and cost considerations.



Section 7 outlines specific open problems and potential research directions in the context of queueing and scheduling for LLM systems.



Section 8 concludes the paper by summarizing the key findings and emphasizing the importance of continued research in this interdisciplinary area.

By bridging the gap between queueing theory and the practical challenges of LLM deployment, we hope to contribute to the development of more efficient, scalable, and cost-effective AI systems. We invite researchers from both fields to engage with the open problems identified and collaborate on solutions that will advance the state of the art in machine learning and queueing systems alike.


\section{Scheduling with Job Size Prediction}


\begin{itemize}
    \item 

Comprehensive Survey: Provide a detailed overview of existing algorithms that use job size predictions for scheduling. Discuss various prediction techniques (e.g., machine learning models, statistical methods) and their accuracy.

    \item
Comparative Analysis: Compare the performance of these algorithms in different scenarios, possibly using metrics like throughput, latency, and resource utilization.

    \item
Challenges in Predictions: Address issues like prediction errors, dynamic workloads, and how they impact scheduling effectiveness.

\end{itemize}


\section{LLM - problem definition}


LLM is not a server

\begin{itemize}
    \item inference time scheduling:  Define key concepts such as inference time scheduling, KV (Key-Value) limited memory, and preemption in the context of LLMs.
    \item Inference Time Scheduling: Discuss how the variable and often substantial inference times of LLMs complicate scheduling.

    \item introduce KV limited memory. KV Limited Memory: Explain how memory constraints affect the processing of large models and the strategies to mitigate these limitations.

    \item  preemption problem when it comes to memory: Preemption Problems: Analyze the difficulties in preempting tasks due to statefulness and the impact on performance metrics like runtime, cost, and accuracy.
    \item performance metrics: run time, cost (\$), accuracy

    \item Visual Aids: Consider adding diagrams or flowcharts to illustrate these concepts and their interrelations.

\end{itemize}



\section{One LLM}


\begin{itemize}
    \item 
Focused Analysis: Examine scheduling and queueing challenges when dealing with a single LLM instance.

    \item 
Optimization Techniques: Discuss strategies to optimize performance, such as batching requests, prioritizing tasks, or adjusting resource allocation dynamically.

    \item 
Case Studies: Include examples or simulations demonstrating the effects of different scheduling algorithms on a single LLM's performance.
\end{itemize}

\section{LLM with API calls}

\begin{itemize}
    \item 
Multi-API Interaction.

    \item 
Memory challenges when it comes to API call 
\end{itemize}



\subsection{Model}
Describe the theoretical underpinnings, assumptions made, and any models or simulations used in your analysis.


\section{Distributed LLM}


\begin{itemize}
    \item Load balancing according to load
    \item Load balancing according to Attention Sharing + load
    \item Load balancing according to Cost + load
\end{itemize}



\begin{itemize}
\item 
Distributed Computing Challenges: Address the complexities introduced by distributing LLM workloads across multiple machines or nodes.

\item 
Load Balancing Strategies:
\begin{itemize}
    \item 
According to Load: Examine traditional load balancing based on current system load and how it applies to LLMs.
    \item 

Attention Sharing + Load: Introduce advanced methods that consider the attention mechanisms in LLMs for more efficient distribution.
    \item 
Cost + Load: Discuss balancing computational cost with performance, including energy consumption and monetary expenses.
\end{itemize}

Scalability Considerations: Analyze how these strategies perform as the system scales and the number of users or requests increases.
\end{itemize}




\paragraph{Open Questions.}

\begin{itemize}
    \item
Preemption overhead presents a challenge in LLM systems (Section~\ref{}). Preemptive scheduling is useful in online settings, where new requests may arrive during the execution of longer requests, allowing interruption of a long-running job to serve a shorter one. However, retaining the KV cache of a preempted job in memory can strain limited resources.

Trail~\cite{} addresses this overhead by modifying SRPT (Shortest Remaining Processing Time). In standard SRPT, any new request with a shorter remaining time preempts the running request. Trail adapts this approach by turning off preemption once a request reaches a certain age, defined as the fraction of its total work completed. For ``young'' requests, the associated KV cache is small, making preemption relatively inexpensive in terms of memory. For ``old'' requests, finishing them frees significant memory more quickly. Trail uses a global threshold, \(c \cdot \text{request size}\), where \(0 \leq c \leq 1\), and preemption is disabled once a request’s age exceeds this threshold. 

A more refined approach to preemption handling could be considered instead of relying on a global threshold, as the KV cache capacity depends on factors such as model size, batch sizes, and the distribution of incoming request sizes.
Managing preemption introduces open questions, such as dynamically adjusting the preemption threshold in real-time based on the sizes of current batch requests.

  \item Each request consists of two stages: a prefill phase and a decode phase. We know the prefill phase size from the prompt, but the decode phase size (output size in tokens) is unknown. In stage 1 (prefill), we have complete information about the subjob size; in stage 2 (decode), we lack this information. One approach is to predict the decode size or assume a known distribution. Even with such information, we must schedule the two-stage requests while accounting for their differing characteristics: the prefill phase is compute-bound and does not benefit from batching, whereas the decode phase is memory-bandwidth-bound and can benefit from larger batch sizes.

    Consider the case where multiple requests share the same total size \(S\), but differ in how \(S\) is split between the prefill and decode phases (e.g., a short prefill with a long decode vs. a long prefill with a short decode). How should we rank these jobs under these constraints?
    
   \item We next consider a split-phase setting, where one set of GPUs handles the prefill phase, and another set handles the decode phase. In many systems, the decode-phase GPUs are “weaker” because the decode phase is memory-bandwidth-bound rather than compute-bound. This setup resembles tandem servers in queueing systems~\ref{MOR book chapter}, but our “servers” (the GPUs) differ in processing speed, adding complexity to scheduling decisions.


   \item Prompts to LLMs now extend beyond simple user questions. To tackle complex tasks, prompt designers often include domain-specific instructions, examples of tool usage, and extensive context, such as textbook chapters. These prompt components frequently repeat across different requests. For instance, a single long document or video may be queried multiple times with varied questions. In tool-augmented LLMs, requests that use the same tool also share tool instructions. Real-world systems, such as Anthropic, report extensive sharing of long prompts. Although shared prompts can make the prefill phase more efficient, they introduce new challenges in scheduling. We must account for repeated prompt segments when ranking requests, which raises an open question: how do we design scheduling policies that prioritize requests based on shared prompt usage? Consider an example of three requests, \(R_1\), \(R_2\), and \(R_3\). Suppose \(R_3\) is small, while \(R_1\) and \(R_2\) share the same long context. A naive ranking might favor the smallest request first, but it may ignore the benefits of combining the shared context for \(R_1\) and \(R_2\). Exploring how to balance these factors highlights is an open question.
\end{itemize}




\begin{itemize}
\item {Majority~\cite{wang2022self}:} This approach involves submitting the same request multiple times (either to the same model instance with different random seeds or temperature settings or across models of varying sizes) and aggregating the candidate responses. The final output is determined via majority voting over these candidates. This approach enhances robustness by mitigating errors from any single inference run.


\item {Rebase~\cite{wu2024inference}:} This approach generates multiple outputs from each prompt, but these outputs represent intermediate reasoning steps rather than final answers. A reward model scores each step, and the highest-scoring nodes are selected as parent nodes for the next expansion. This iterative process builds a tree of reasoning steps, with the final answer produced either by weighted majority voting or by selecting the highest-scored candidate.

\item {Monte Carlo Tree Search~\cite{feng2023alphazero, hao2023reasoning}:} This approach iteratively constructs a solution tree starting from each prompt. In each iteration, it expands a node by sampling a continuation from the LLM until reaching a leaf node with a candidate solution. The candidate's score is then back-propagated to update its ancestors' scores. After multiple iterations, MCTS effectively explores both deeper and broader portions of the solution space.

\item {Internalized Chain-of-Thought:} Modern LLMs like OpenAI's o1~\cite{openai_o1}, Qwen-QWQ~\cite{qwq}, and Deepseek r1~\cite{guo2025deepseek} have been trained to internalize reasoning.
These models generate extended chain-of-thought~\cite{wei2022chain} sequences, which enhance the reasoning capabilities of LLMs by generating intermediate steps that guide the final answer. The reasoning model iteratively refines its output by reflecting on previous tokens until reaching a final answer, with the total number of tokens generated directly corresponding to inference-time compute.
\end{itemize}




%%%%%%%%%%%%%%%%%%%%%%%%%%% EDIT  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Scheduling \emph{two-stage requests}, each consisting of prefill and decode phases presents a challenge. 
%Although the prefill size is fully known from the prompt, the decode size remains unknown and might require a predicted estimate. Complicating matters further, the prefill phase is compute-bound and gains little from batching, whereas the decode phase is heavily memory-bandwidth-bound and can benefit substantially from batching.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/figures/tikz-macros.tex <==
\makeatletter

% Prelude sets $ to active, but calc needs it as math shift.
%\catcode`\$=3 % math shift
\catcode`\$=13 % active %RANA

\usetikzlibrary{backgrounds, math, shapes, shapes.arrows, positioning,
  decorations.markings, decorations.pathreplacing, calligraphy}

\tikzset{
  bgbox/.style={framed, background rectangle/.style={fill=black!7, rounded corners=1em}},
  figure/.style={x=\xscale, y=\yscale, semithick, font=\footnotesize, bgbox},
  axis/.style={thin},
  guide/.style={thin, black!30, dashed},
  srpt-b/.style={ultra thick, color=orange!60!yellow!80!black},
  srpt-se/.style={ultra thick, color=cyan!75!blue!90!black},
  psjf-e/.style={ultra thick, color=green!30!yellow!70!black},
  srpt-e/.style={ultra thick, color=magenta!45!blue!70!white},
  psjf/.style={ultra thick, color=green!60!blue!85!black},
  srpt/.style={ultra thick, color=magenta!60!red!85!black},
  size/.style={line width=2pt, color=magenta!75!blue!90!white},
}

\def\@above{above}
\def\@below{below}
\def\@negative{-}
\newcommand{\downmode}{%
  \def\@above{below}
  \def\@below{above}
  \def\@negative{}}

\newcommand{\xscale}{7}
\newcommand{\yscale}{7}
\newcommand{\ticksize}{3}
%\newcommand{\arrowsize}{5} %RANA
\renewcommand{\arrowsize}{5}

\newcommand{\xarrowsize}{(\arrowsize/\xscale)}
\newcommand{\yarrowsize}{(\arrowsize/\yscale)}

\newcommand{\projx}[1]{($ (0,0)!#1!(1,0) $)}
\newcommand{\projxheight}[2]{($ (0,#2)!#1!(1,#2) $)}
\newcommand{\midpt}[2]{($ #1!0.5!#2 $)}

\newcommand{\xguide}[3][]{%
  \draw[axis] ({#2}, 0) -- ({#2}, {\@negative(\ticksize)/\yscale})
  node[\@below] {\ifempty{#1}{$#2$}{#1}\vphantom{by}};
  \draw[guide] ({#2}, 0) -- ({#2}, {#3});}
\newcommand{\yguide}[3][]{%
  \draw[axis] (0, {#3}) -- (-\ticksize/\xscale, {#3})
  node[left] {\ifempty{#1}{$#3$}{#1}};
  \draw[guide] (0, {#3}) -- ({#2}, {#3});}
\newcommand{\yguidenolabel}[2]{%
  \draw[guide] (0, {#2}) -- ({#1}, {#2});}

\newcommand{\axes}[6]{%
  \draw[axis, ->] (-\ticksize/\xscale, 0)
  node[left] {#3\vphantom{by}} -- ({#1 + \xarrowsize}, 0) node[right] {#4\vphantom{by}};
  \draw[axis, ->] (0, \@negative\ticksize/\yscale)
  node[\@below] {#5\vphantom{by}} -- (0, {#2 + \yarrowsize})
  node[\@above] {#6\vphantom{by}};}

% Set $ back to active for prelude
\catcode`\$=13 % active
\makeatother


==> sections/figures/tikz-macros_new.tex <==
\makeatletter
% Remove the catcode changes for '$' to avoid conflicts with acmart.
% (The following lines are removed)
% \catcode`\$=3 % math shift

% Either remove this if you already loaded the libraries in your preamble...
\usetikzlibrary{backgrounds, math, shapes, shapes.arrows, positioning, 
  decorations.markings, decorations.pathreplacing, calligraphy}
% ...or comment it out if you prefer to load all TikZ libraries in one spot.

\tikzset{
  bgbox/.style={framed, background rectangle/.style={fill=black!7, rounded corners=1em}},
  % Note: The style name "figure" here is used for TikZ; it is not the same as the "figure" environment.
  figure/.style={x=\xscale, y=\yscale, semithick, font=\footnotesize, bgbox},
  axis/.style={thin},
  guide/.style={thin, black!30, dashed},
  srpt-b/.style={ultra thick, color=orange!60!yellow!80!black},
  srpt-se/.style={ultra thick, color=cyan!75!blue!90!black},
  psjf-e/.style={ultra thick, color=green!30!yellow!70!black},
  srpt-e/.style={ultra thick, color=magenta!45!blue!70!white},
  psjf/.style={ultra thick, color=green!60!blue!85!black},
  srpt/.style={ultra thick, color=magenta!60!red!85!black},
  size/.style={line width=2pt, color=magenta!75!blue!90!white},
}

\def\@above{above}
\def\@below{below}
\def\@negative{-}
\newcommand{\downmode}{%
  \def\@above{below}%
  \def\@below{above}%
  \def\@negative{}%
}

\newcommand{\xscale}{7}
\newcommand{\yscale}{7}
\newcommand{\ticksize}{3}
\newcommand{\arrowsize}{5}


\newcommand{\xarrowsize}{(\arrowsize/\xscale)}
\newcommand{\yarrowsize}{(\arrowsize/\yscale)}

\newcommand{\projx}[1]{($ (0,0)!#1!(1,0) $)}
\newcommand{\projxheight}[2]{($ (0,#2)!#1!(1,#2) $)}
\newcommand{\midpt}[2]{($ #1!0.5!#2 $)}

\newcommand{\xguide}[3][]{%
  \draw[axis] ({#2}, 0) -- ({#2}, {\@negative(\ticksize)/\yscale})%
  node[\@below] {\ifstrempty{#1}{$#2$}{#1}\vphantom{by}};%
  \draw[guide] ({#2}, 0) -- ({#2}, {#3});%
}
\newcommand{\yguide}[3][]{%
  \draw[axis] (0, {#3}) -- (-\ticksize/\xscale, {#3})%
  node[left] {\ifstrempty{#1}{$#3$}{#1}};%
  \draw[guide] (0, {#3}) -- ({#2}, {#3});%
}
\newcommand{\yguidenolabel}[2]{%
  \draw[guide] (0, {#2}) -- ({#1}, {#2});%
}

\newcommand{\axes}[6]{%
  \draw[axis, ->] (-\ticksize/\xscale, 0) node[left] {#3\vphantom{by}} --
    ({#1 + \xarrowsize}, 0) node[right] {#4\vphantom{by}};%
  \draw[axis, ->] (0, \@negative\ticksize/\yscale) node[\@below] {#5\vphantom{by}} --
    (0, {#2 + \yarrowsize}) node[\@above] {#6\vphantom{by}};%
}

% Remove the following line so that the math shift catcode remains standard.
% \catcode`\$=13 % active

\makeatother


==> sections/removed.tex <==
\begin{figure}[ht]
\centering
\begin{tikzpicture}[node distance=2cm, auto]
    % Nodes
    \node (input) [draw, rectangle] {Input Query};
    \node (stage1) [draw, rectangle, below of=input] {Stage 1: Reasoning Step};
    \node (decide) [draw, diamond, below of=stage1, aspect=2, inner sep=2pt] {Continue?};
    \node (stage2) [draw, rectangle, below left of=decide, node distance=3cm] {Stage 2: Reasoning Step};
    \node (stageN) [draw, rectangle, below of=stage2] {Stage N: Reasoning Step};
    \node (output) [draw, rectangle, below right of=decide, node distance=3cm] {Final Answer};
    
    % Arrows
    \draw[->] (input) -- (stage1);
    \draw[->] (stage1) -- (decide);
    \draw[->] (decide) -- node[left]{Yes} (stage2);
    \draw[->] (stage2) -- (stageN);
    \draw[->] (stageN) -- node[left]{No} (output);
    \draw[->] (decide.east) -- node[right]{No} ++(1,0) |- (output);
\end{tikzpicture}
\caption{Chain-of-thought scheduling: at each stage, the scheduler decides whether to continue reasoning or to return the final answer.}
\label{fig:chain_of_thought}
\end{figure}

\begin{figure}[ht]
\centering
\begin{tikzpicture}[node distance=1.8cm, auto]
    % Input node common to both approaches
    \node (input) [draw, rectangle] {Input Query};
    \node (split) [draw, circle, below of=input, inner sep=1pt] {Split};
    
    % Majority Voting Branch
    \node (majLabel) [below left of=split, node distance=2.5cm] {Majority Voting};
    \node (maj1) [draw, rectangle, below of=majLabel] {Inference Run 1};
    \node (maj2) [draw, rectangle, below of=maj1] {Inference Run 2};
    \node (maj3) [draw, rectangle, below of=maj2] {Inference Run 3};
    \node (consensus) [draw, rectangle, below of=maj3] {Consensus};
    
    % Chain-of-Thought Branch
    \node (cotLabel) [below right of=split, node distance=2.5cm] {Chain-of-Thought};
    \node (cot1) [draw, rectangle, below of=cotLabel] {Stage 1: Reasoning};
    \node (cot2) [draw, rectangle, below of=cot1] {Stage 2: Reasoning};
    \node (cotOut) [draw, rectangle, below of=cot2] {Final Answer};
    
    % Connections
    \draw[->] (input) -- (split);
    \draw[->] (split) -- (majLabel);
    \draw[->] (split) -- (cotLabel);
    
    \draw[->] (majLabel) -- (maj1);
    \draw[->] (maj1) -- (maj2);
    \draw[->] (maj2) -- (maj3);
    \draw[->] (maj3) -- (consensus);
    
    \draw[->] (cotLabel) -- (cot1);
    \draw[->] (cot1) -- (cot2);
    \draw[->] (cot2) -- (cotOut);
\end{tikzpicture}
\caption{Comparison of majority voting (ensemble inference with consensus) and chain-of-thought reasoning (sequential multi-stage process).}
\label{fig:comparison}
\end{figure}


\begin{figure}[ht]
\centering
\begin{tikzpicture}[node distance=2cm, auto]
    % Nodes
    \node (start) [draw, rectangle] {Input Query};
    \node (evaluate) [draw, rectangle, below of=start] {Evaluate Intermediate Output};
    \node (decision) [draw, diamond, below of=evaluate, aspect=2, inner sep=2pt] {Promising Trajectory?};
    \node (allocate) [draw, rectangle, below left of=decision, node distance=3cm] {Allocate More Resources};
    \node (preempt) [draw, rectangle, below right of=decision, node distance=3cm] {Preempt and Reassign};
    \node (final) [draw, rectangle, below of=decision, node distance=4cm] {Return Final Answer};
    
    % Arrows
    \draw[->] (start) -- (evaluate);
    \draw[->] (evaluate) -- (decision);
    \draw[->] (decision) -- node[left]{Yes} (allocate);
    \draw[->] (decision) -- node[right]{No} (preempt);
    \draw[->] (allocate) |- (final);
    \draw[->] (preempt) |- (final);
\end{tikzpicture}
\caption{Resource allocation flowchart for adaptive scheduling based on intermediate reasoning outputs.}
\label{fig:resource_allocation}
\end{figure}



% Predictions come with a computational cost, and they have various forms. Some predictions classify jobs as short or long based on a predefined threshold. Others estimate service times directly using regression techniques, while a third type predicts the entire service time distribution. Each approach adds its own overhead. This raises the question of whether resources spent generating predictions might sometimes be better used to process the jobs directly. 
% The work in~\cite{} shows that even a 1bit prediction, classifying a job as short or long, followed by applying a First-Come-First-Serve (FCFS) policy within each category, can improve scheduling and minimize response time \rana{define response time}. Building on this, SkipPredict~\cite{} is the first approach to explicitly account for the inherent cost of predictions in scheduling. Instead of uniformly applying detailed service time predictions to every job, SkipPredict adopts a two-tier strategy. It first uses a 1bit, cheap prediction, to classify jobs as short or long. The scheduler then prioritizes jobs predicted to be short and schedules them as FCFS, while for those predicted to be long, SkipPredict applies a second round of more detailed (service time prediction) computationally intensive predictions to approximate the Shortest Remaining Processing Time policy (SPRPT).




\subsubsection{GPU Resource Allocation and Load Balancing}


\begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.35\linewidth}
        \centering
        \includegraphics[width=\linewidth]{sections/figures/shared_phases.drawio.pdf}
        \caption{Pooled GPUs}
        \label{fig:pooled_gpus}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.35\linewidth}
        \centering
        \includegraphics[width=\linewidth]{sections/figures/split_phase.drawio.pdf}
        \caption{Dedicated GPUs for prefill and decode}
        \label{fig:dedicated_gpus}
    \end{subfigure}
    \caption{GPU organizations: comparing pooled GPUs with dedicated GPUs for prefill and decode phases.}
    \label{fig:gpus_organization}
\end{figure}


\noindent{{\bf Open Questions:}}
\begin{itemize}
\item
    An interesting open problem arises when considering how to orchestrate GPU resources, which may differ in computation and memory, across different architectural organizations (as illustrated in Figure~\ref{fig:gpus_organization}). For instance, GPUs suited for \emph{decode} might favor larger memory and relatively lower compute throughput, while GPUs suited for \emph{prefill} might prioritize higher compute throughput at lower memory footprints. In the \emph{pooled GPUs} approach, each GPU handles both the prefill and decode phases. After completing the prefill phase, a request can either proceed directly to decoding on the same GPU or re-enter the queue to be processed by any available GPU. The latter option poses a challenge: transferring the KV cache from the prefill GPU to the decode GPU and storing the KV cache until a decode GPU is assigned introduces memory and communication overhead. This raises the question: \emph{should we complete the request immediately or preempt it and rank it among waiting requests?}. 
    A key challenge here is to design the best scheduling policy to optimize utilization and latency. In contrast, \emph{dedicated GPUs} splits the fleet into separate groups: one exclusively handles prefill, the other decodes. This arrangement looks similar to tandem servers in queueing systems~\cite{}, but in our case, the GPUs differ 
    in speed, and there is KV cache transfer overhead, making scheduling more complex. While this can mitigate conflicts within each phase, it risks underutilizing one subset if the workload distribution is imbalanced (for example, when large prompt sizes prolong prefill while decoding resources remain idle). Determining how to best allocate and schedule these resources in both scenarios remains an open research question.

\item

    Beyond determining the optimal GPU organization, further gains may be achieved by incorporating additional factors like prompt overlap into scheduling decisions. Repeated prompts can reduce the cost of the prefill phase when requests sharing the same context are batched, but it remains unclear how best to order such requests. For instance, consider three requests \(R_1\), \(R_2\), and \(R_3\), where \(R_3\) is small and \(R_1\) and \(R_2\) share a long context. A naive strategy might always prioritize the smaller \(R_3\), but this approach misses the opportunity to batch \(R_1\) and \(R_2\). Future research must develop and analyze adaptive algorithms that continually weigh prompt overlap, real-time GPU load, and queue dynamics to minimize latency and resource underutilization. Theoretical modeling and trade-off analysis of these multi-factor schedulers represent an important open challenge in large-scale LLM deployments.
\end{itemize}







\subsubsection{Cost and Hardware Trade-offs}

Scheduling policies for large-scale LLM deployment typically focus on latency or throughput goals, often overlooking cost optimization. Yet, in practice, operating budgets and usage-based billing models can significantly impact system design. 
    
\noindent{{\bf Open Questions:}}
\begin{itemize}
\item
    Integrating financial considerations into scheduling algorithms leads to natural multi-objective optimization formulations that simultaneously target low latency and low cost. This raises further questions: 
    
    \begin{itemize}
        \item \emph{Budget-Constrained Scheduling:} How can we devise scheduling and resource-allocation strategies that respect a global cost target while ensuring acceptable response times?
    
        \item \emph{Adaptive Multi-Objective Policies:} Given that latency and cost trade-offs vary with workload and SLA requirements, is there a unified, adaptive approach that prioritizes one objective under certain conditions while shifting emphasis to the other as constraints or user demands evolve?
    \end{itemize}



%Alongside these multi-objective scheduling challenges, 

\item 
another key question is how hardware choices influence the overall cost–latency trade-off. An interesting open problem is whether we can systematically estimate how many lower-capacity GPUs, each with limited memory and throughput, are needed to match or exceed the performance of a single high-end GPU in LLM inference. Beyond raw throughput measurements, the comparison involves analyzing communication overhead between multiple smaller devices, the availability (and cost) of high-bandwidth interconnects, and the cumulative power draw. These factors can degrade the apparent cost benefits of scaling out. Developing theoretical models and empirical studies of this trade-off would clarify the conditions under which investing in a single, more capable GPU is preferable to assembling a larger cluster of smaller GPUs—particularly for the prefill and decode phases of LLM workloads.

%In addition to the inherent trade-offs between cost and latency, 

\item 
dynamic hardware availability further complicates scheduling decisions in large-scale LLM deployments. In many practical settings, additional GPUs become available only after an LLM service is already operational. The primary challenge is to integrate these resources without disrupting ongoing workloads and to decide whether they should support the prefill phase (improving large prompt handling) or the decode phase (reducing response times for interactive queries). The system’s current bottlenecks, workload composition, and cost constraints may differ from the original design assumptions, making naive allocations suboptimal. Future research directions include developing methods to dynamically identify resource-starved phases and formulating scheduling or load-balancing algorithms that adapt to changing GPU availability. Prediction of request arrival rates and prompt sizes can guide which phase to enhance at any given moment. Another approach is adjusting resource assignments when newly added GPUs differ from existing ones in memory capacity, compute throughput, or cost. 

\end{itemize}

\subsection{Balancing Interactive and Non-Interactive Workloads}

\noindent{{\bf Open Questions:}}
\begin{itemize}
\item
A key open challenge arises from handling requests with differing latency requirements. Interactive (chat) requests demand near-immediate responses, whereas long-running or batch-style requests can tolerate delay but must not be starved. Although prioritizing short, user-facing queries ensures responsiveness, it risks indefinitely postponing larger tasks—especially under high load. This tension raises critical questions about how best to assign and adapt scheduling policies.
The ultimate goal is to develop scheduling algorithms that deliver low-latency service for interactive queries without compromising the progress and quality of non-interactive workloads, even under highly variable load conditions. This challenge can be framed within a multi-objective scheduling framework that balances latency with fairness, and insights from queueing theory may offer guarantees to prevent starvation.
\end{itemize}











%======= LLM reasoning can be approached using two distinct methodologies. The first, majority voting~\cite{}, involves submitting the same request multiple times (either to the same model instance or across models of varying sizes) and aggregating the candidate responses to derive a consensus answer. This ensemble approach enhances robustness by mitigating errors from any single inference run, 


yet it also introduces scheduling challenges and opportunities. In particular, coordinating parallel inference tasks demands a scheduler capable of balancing the additional computational overhead against the improved reliability and accuracy offered by consensus-based decision-making.


%The second approach is chain-of-thought reasoning~\cite{}, which enhances the reasoning capabilities of LLMs by generating intermediate steps before arriving at a final answer. This approach extends LLM inference into a multi-stage process, where the generation of intermediate tokens reveals the model's internal decision-making and guides the final response.

The sequential and often recursive nature of chain-of-thought reasoning introduces unique challenges and opportunities for scheduling. Unlike traditional LLM serving, where scheduling decisions focus primarily on token-level throughput and latency, chain-of-thought


reasoning requires adaptive scheduling that responds to the dynamic state of the reasoning process. At each step, the scheduler must decide whether to allocate additional resources to generate further reasoning steps or to terminate the process and return a final answer. This decision depends on factors such as the complexity of the input prompt (i.e., the predicted depth of reasoning needed), the current system load, and the allocated cost budget for the request. Moreover, some queries may require only a few steps before settling on a solution, while others might necessitate extensive exploration, leading to execution times that traditional scheduling algorithms are not designed to handle. In these systems, the notion of request size extends beyond the output token count to include the number of reasoning steps required for convergence. This information may be predicted and used to inform scheduling decisions.
